Protocols for Checking Compromised Credentials

To prevent credential stuffing attacks, industry best practice now proactively checks if user credentials are present in known data breaches. Recently, some web services, such as HaveIBeenPwned (HIBP) and Google Password Checkup (GPC), have started providing APIs to check for breached passwords. We refer to such services as compromised credential checking (C3) services. We give the first formal description of C3 services, detailing different settings and operational requirements, and we give relevant threat models. One key security requirement is the secrecy of a user's passwords that are being checked. Current widely deployed C3 services have the user share a small prefix of a hash computed over the user's password. We provide a framework for empirically analyzing the leakage of such protocols, showing that in some contexts knowing the hash prefixes leads to a 12x increase in the efficacy of remote guessing attacks. We propose two new protocols that provide stronger protection for users' passwords, implement them, and show experimentally that they remain practical to deploy.

==> experiment.tex <==
\subsection{Evaluation}
\label{sec:eval}
To evaluate the performance of Algorithms \ref{alg:truncation_calculation} and \ref{alg:similar_prefix}, we build an implementation that processes \cite{haveibeenpwned}, a  list of over 320 million leaked passwords. The passwords already come hashed using the SHA1 algorithm, saving a step.

With the hashed passwords collected in a simple text file, the hashes are pre-processed to ensure all the values are unique and additionally to sort the hashes into ascending alphabetical order such that Algorithm \ref{alg:truncation_calculation} can work effectively. The output of this pre-processing is passed into a text file which contains the $320,335,236$ hashes.

An implementation is created for Algorithm \ref{alg:truncation_calculation} which works by starting up one process which reads hashes piped into the program and passes them down a channel. A separate worker process then iterates through the values in the channel and calculates how similar the prefix of any individual hash is to any other hash in the data set. Any time a given hash has a common prefix which is shorter in length than the previous shortest common prefix, the value is recorded. After the program has finished execution we find out the shortest common prefix between any two hashes for the entire list of hashes.

Note that we concurrently read hashes from the text file into the channel, whilst running the worker to run calculations. As the file containing all the hashes measures around $13GB$ it is impractical on most computers to load the entire file into memory prior to processing. As a result, we feed the contents of the file into a channel and the worker processes the values as they are loaded, thus reducing the amount of hashes that need to be stored in memory at a particular time.

With the Hash Prefix Length determined, it is then possible to run Algorithm \ref{alg:populate} to actually group together hashes by their prefix. The simplest implementation for this would be to write a text file for each Hash Prefix containing a list of all hashes associated to that prefix. For instance; a file called $19FCF.txt$ would create all hashes starting with $19FCF$.

At first glance, this seems like an elegant and practical solution. These files could be placed on a web server in static format, then when a third party wishes to run a query on the basis of a given Hash Prefix, they simply send a HTTP query for where the file should exist (e.g. $example.com/191FCF.txt$) and if the file exists, the client checks to see if any of the hashes within the text file match the local hash.

This approach can rapidly become impractical as the Hash Prefix increases in size. As hexadecimal contains 16 distinct symbols, the total amount of possible files where the hash prefix is 4 characters long is $16^4 = 65,536$. This seems manageable, but when the Hash Prefix is increased to 5, $16^5 = 1,048,576$ and when the Hash Prefix is raised to 6 the total possible amount of files becomes $16^6 = 16,777,216$. File management tools can struggle to handle such a vast quantity of files and, without adopting a directory structure, File Systems can even reach their limit for the number of files in a single directory.

As an alternative, it is possible to create a simple 2 column database structure which connects Hash Prefixes to individual hashes. For the database system, our implementation used SQLite which acts as an embedded database with all the data stored in a single file. As a hash should only need to be stored once throughout the database, a unique property can be applied to the database column. Additionally to accelerate the searching of hashes when querying by the Hash Prefix, an index can be set-up on the Hash Prefix column.

\paragraph{Results.} Upon running Algorithm \ref{alg:truncation_calculation} on \cite{haveibeenpwned}, the ideal Minimum Hash Prefix size was found to be 5. Comparison of the first 2 hashes found the common Hash Prefix size to be 8, though this incrementally decreased to 7, then 6 and eventually 5 as the data set was processed further.

We therefore set the Hash Prefix size to 5 when running \ref{alg:populate}. Splitting the hashes into buckets would mean a maximum of $16^5 = 1,048,576$ buckets would be utilized, assuming that every possible Hash Prefix would contain at least one hash. In the final data set we found this to be the case and the amount of distinct Hash Prefix values was equal to the highest possible quantity.

The Hash Prefix $EDC9E$ had the fewest amount of hashes associated to it at 215 hashes, by contrast the Hash Prefix with the largest amount of hashes associated to it was $00000$ which had 420 hashes associated to it. The median amount of hashes associated to a given Hash Prefix was 305, the mean number was also 305.

The Hash Prefix $00000$ contained 25 more hashes than the second largest Hash Prefix ($2456B$ which was associated to 395 hashes). It can be expected for the $00000$ Hash Prefix to contain the most amount of hashes, as the small hash values are left-padded with $0$s to ensure the hexadecimal strings are 40-characters long. Despite this, the largest hash bucket was only 95\% larger than the smallest, with the largest Hash Prefix still containing few enough hashes for relatively fast computational evaluation.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> implementation.tex <==
\subsection{Implementation of {\hibp}}
\label{sec:implementation}
For our implementation; we seek to provide an API service which allows remote web services and clients to validate whether a password is or is not in a database of leaked passwords, without ever needing to send the password itself. In order to achieve this anonymity, a range query can be used such that the client will request all passwords in a particular range. This range will send back multiple results, from here the client is able to determine if one of the passwords that is returned is identical to the password supplied by the user. An interceptor the operator of the API service cannot themselves tell if the queried password is in the database itself or not, as the only query was for a range of data.

\paragraph{Mitigating Background Knowledge Attacks.} In anonymising text data, it is possible to infer attributes about the contents based on the search query. For example; a search request is put to the API service for all leaked passwords starting with "8StJoh" and it is known the requester resides at the address "8 St Johns Road", it is possible to infer the password even if it is not in the database of leaked passwords itself. This is a known restriction in $k$-anonymity and has been discussed extensively in \cite{Machanavajjhala:2007:LDP:1217299.1217302} where $l$-diversity is proposed in order to help mitigate such Background Knowledge Attacks. As such, it is important to ensure the ranges of passwords queried do not become quasi-identifier attributes themselves.

As a result of the Avalanche Effect, by hashing every password we are able to ensure that hashes which are similar are not generated from similar plain-texts. As such, we simply run every plain-text password in the database through the SHA1 algorithm which is known to maintain the Avalanche Effect property \cite{yang2015improved}.

Note that unlike when passwords are normally hashed, the aim here is not to ensure that the hashed passwords cannot be restored to their plain-text which is why the hashing has been done without any salting or using ordinarily password derivation functions like BCrypt \cite{provos1999bcrypt}. The plain-text values of these passwords is already known as they have been previously leaked and uniquely salting the passwords would make it impractical for them to be searched.

\paragraph{Distributing Hashes into Buckets.} For hashes to be able to be easily queried by third-party services, they are split into buckets which consist of a set of hashes. Let $S = \{h_1, h_2, h_3, \ldots, h_S\}$ where $S$ represents a set of password hashes and let $l$ represent the minimum amount of hashes in an individual bucket. Our aim is to find $A = \{b_1, b_2, b_3, \ldots, b_n\}$ such that $b_n \subset S$ whilst $\sum_{n=1}^{|A|} b_n = |S|$ and $|b_n| \geq l$.

\cite{friedman2006k} discusses how a decision tree can be used for searching a dataset whilst maintaining $k$-anonymity. In this instance, as we are anonymising 1-dimensional data, it is possible to implement a tree structure to allow third-parties to search for password hashes so long as any search query will return a multiple hashes.

Take the example of a crude theoretical hashing algorithm that produces it's output as an integer between $1$ and $30$, with the breached hash values are stored in a decision tree of a similar structure to Fig. \ref{fig:tree}. The service is exposed via an online API service; when a consumer wishes to run a query to check whether a given hash is in the database, they will first submit an API to call an endpoint which provide the range of hashes available in the database and will state which questions to answer in order to continue the search. This decision tree will continue until the query achieves it's desired level of accuracy at which point the complete set of hashes matching that query is returned.

\begin{figure}[h]
\Tree[.1$\leq$n$\leq$30 [.$\leq$15 [1,2,5,7,14,15 ]]
          [.$>$15 [.$\leq$23 [16,17,20,23 ] ]
                [.$>$23 [.24,27,30 ]]
		     ]
		]
\caption{Example Decision Tree}
\label{fig:tree}
\end{figure}

As the number of hashes stored in the decision tree increases, in order reduce the amount of values returned by the leaf nodes, the depth of the decision tree must also increase. B-Tree is a simple example of a decision tree; with $n$ items, the longest path of a B-Tree of order $d$ is at most $\log_d n$ nodes \cite{comer1979ubiquitous}. Whilst $log n$ difficulty can be considered small for many applications, it is important to note that at each decision point an API call will need to be made. With low latency being a key concern (such as in developing countries or for those over mobile connections), this approach was not suitable.

A similar approach could be to provide a map file which flattens a tree structure into a single index file, an example of the data tree Fig. \ref{fig:tree} represented in a flat file format is demonstrated in Fig. \ref{fig:flatten_tree}. 

\begin{figure}[h]
\begin{mdframed}
1.txt: $1 \leq n \leq 15$

2.txt: $15 \leq n \leq 23$

3.txt: $23 \leq n \leq 30$
\end{mdframed}
\caption{Example Flattened Tree}
\label{fig:flatten_tree}
\end{figure}

As hashes of a greater range are added, instead of the tree depth increasing, instead the size of the index file would increase. In other words, we'd simply be trading a large amount of API requests for a less, but significantly larger, index file. Decreasing the index file would require an increase the order of the tree itself (thereby increasing the amount of hashes stored in an individual leaf). As a result this solution also seemed impractical.

By allowing the client to independently calculate the size of a given chunk (and discover which chunk file it should look for), we would eliminate the need for there to be a tree entirely. Instead the client would itself know where to look to find hashes in a given range. 

\begin{figure}[h]

\begin{mdframed}
Start: 5

End: 25

Step: 5
\end{mdframed}
\caption{Example Index File}
\label{fig:index_file}
\end{figure}

One mechanism of doing this would be through performing arithmetic operations on the hashes. Firstly the database is pre-processed by calculating the minimum value of the hash alongside the maximum value. From here, a step value is calculated which we calculate the maximum distance between $l$ values in the entirety of the data set, this becomes our $step$ value. This data is presented in an index file for the API, an example structure is shown in Fig. \ref{fig:index_file}. In order to determine which hashes are then split into which files, a simple algorithm is used: $\lfloor(largestHash-smallestHash)/step\rfloor+1$.

When a client wishes to check if their hash is in a given database, they can work out which file to look in by re-running the algorithm on the client side with the appropriate values provided by the APIs index file. Whilst this approach seems promising, there is still a significant drawback. Hashes typically are large numbers, outside the maximum integer value of a variety of programming languages and as such, developers would need to implement Big Integer libraries to perform such calculations.

A simpler alternative to anonymize hash data is to instead truncate the hashes such that the a query is made to an API service on the basis of prefix of a hash. This idea is not completely novel, this concept is briefly discussed in \cite{lu2010towards} and \cite{manweiler2009smile}. \cite{lu2010towards} proposes an alternative Domain Name System for the Internet which utilizes Distributed Hash Tables. In essence, clients retrieve all values whose hash value matches a Hash Prefix, thereby achieving anonymity. \cite{manweiler2009smile} also discusses the utilization of Hash Prefixes to preserve k-anonymity when sending messages in location-based social networks. Neither of these concepts are relevant to the anonymization of password hashes and therefore the work in determining the prefix length is not applicable to this use-case. Additionally, there has been little work done to determine the distribution of hashes depending on a prefix. 

This approach can be implemented in a relatively simple way. Suppose a user enters the password $test$ into a login form and the service they're logging into is programmed to validate whether their password is in a third-party database of leaked password hashes. Firstly the client will generate a hash (in our case using SHA1) of $a94a8fe5ccb19ba61c4c0873d391e987982fbbd3$. The client will then truncate the hash to a predetermined number of characters (for example, 5) resulting in a hash prefix of $a94a8$. This hash prefix is then used to query the remote database for all hashes starting with that prefix (for example, by making a HTTP request to $example.com/a94a8.txt$). The entire hash list is then downloaded and each downloaded hash is then compared to see if any match the locally generated hash. If so, the password is known to have been leaked.

\paragraph{Determining Hash Prefix Length.} A critical decision to make, prior to anonymising data, is the length of the Hash Prefix that is used for clients to be able to search the database. For a range of password hashes to hold the property of $l$-diversity, there must be at least $l$ distinct password hashes which start with the same Hash Prefix. When every Hash Prefix in the entire password database holds the property of $l$-diversity, the entire database can be said to have $l$-diversity \cite{li2007t}.

Algorithm \ref{alg:truncation_calculation} demonstrates a simple algorithm to find a Hash Prefix length that ensures every Hash Prefix represents at least more than one hash from the entire dataset. This algorithm uses a method defined in Algorithm \ref{alg:similar_prefix} for determining the similar prefix between two individual hashes. The first step Algorithm \ref{alg:truncation_calculation} performs is order all hashes in alphabetical order, this allows for rapid checking to find the similarity in the prefix of two hashes as the program only needs to look at two other values instead of searching the entire text to locate another hash with the same prefix. This property helps save memory utilization when dealing with large sets of hashes.

\begin{algorithm}
 \KwData{passwordHashes}
 \KwResult{prefixLength}
 $S$ = \{\}\;
 prefixLength = 40\;
 \tcp{Default prefix length set to SHA1 hash length}
 passwordHashes = sortAlphabetically(passwordHashes)
 \While{passwordHashes as hash}{
  $S_n$ = hash\;
  \If{$|S|$ == 3}{
    A = similarPrefix($S_1$, $S_2$)\;
    B = similarPrefix($S_2$, $S_3$)\;
    similarity = max(A, B)\;
    \If{similarity $<$ prefixLength}{
      prefixLength = similarity\;
    }
   delete($S_1$)\;
   }
 }
 \label{alg:truncation_calculation}
 \caption{Calculate Truncation to Anonymise Hashes}
\end{algorithm}

\begin{algorithm}
 \SetKwFunction{FSimilarPrefix}{SimilarPrefix}
 \SetKwProg{Pn}{Function}{:}{\KwRet}
  \Pn{\FSimilarPrefix{$a$, $b$}}{
    \For{length = 0; length $\leq$ length(a); length+1}{
      aPrefix = truncate(a, length)\;
      bPrefix = truncate(b, length)\;
        \If{aPrefix == bPrefix}{
          similarity = length\;
          continue\;
        }
        break\;
    }
    return similarity\;
  }
 \label{alg:similar_prefix}
 \caption{Similar Prefix Method}
\end{algorithm}

\subsection{Distributing Hashes into Buckets by Prefix}

With the Hash Prefix length determined, we use Algorithm \ref{alg:populate} to group every password hash together by their respective Hash Prefix. This algorithm takes input with a set of password hashes and the desired truncation length that's required.

\begin{algorithm}
 \KwData{passwordHashes, truncationLength}
 \KwResult{results}
 $results$ = \{\}\;
 \While{passwordHashes as hash}{
  $n$ = truncate(hash, truncationLength)\;
  \tcp{Hash Prefix is stored in $n$}
  $results_{n}$.insert(hash)\;
  \tcp{Hash Prefix ($n$) stored in $results$ set, with individual hashes stored as a $subset$ (in $result_n$)}
 }
 \label{alg:populate}
 \caption{Generate Anonymised Hash Information}
\end{algorithm}

In Algorithm \ref{alg:populate}, we create a set $results$ which contains Hash Prefix values. Each of these Hash Prefix values act as sets which then contain a subset consisting of the hashes associated to the relevant Hash Prefix.

\paragraph{Open Questions. } We have covered a theoretical approach for performing a Range Query by using a Hash Prefix; however, there still remain a number of open questions. Consider the distribution of the hashes, if password hashes are overwhelmingly more likely to start with a particular hash string than others, this leaves potential for a number of problems. A Range Query which returns a small amount of hashes for for one prefix may instead return a vast number of prefixes for another Hash Prefix. If this is the case, we would have to consider an implementation approach which also utilized an alternative mechanism for further filtering (such as a Decision Tree). In order to evaluate whether distribution is a problem, we can evaluate the implementation on a trial data set.




